Replication of arbitrary hole-free shapes via self-assembly with signal-passing tiles

In this paper, we investigate the abilities of systems of self-assembling tiles which can each pass a constant number of signals to their immediate neighbors to create replicas of input shapes. Namely, we work within the Signal-passing Tile Assembly Model (STAM), and we provide a universal STAM tile set which is capable of creating unbounded numbers of assemblies of shapes identical to those of input assemblies. The shapes of the input assemblies can be arbitrary 2-dimensional hole-free shapes. This improves previous shape replication results in self-assembly that required models in which multiple assembly stages and/or bins were required, and the shapes which could be replicated were more constrained, as well as a previous version of this result that required input shapes to be represented at scale factor 2.

==> corner-gadgets.tex <==
\subsection{Description of the frame building tile set}\label{sec:corner-gadgets}

In this section we describe the $\cgSE$ used in our construction.
Figure~\ref{fig:secgCases} shows the $6$ different tile location where the tiles of a $frame$ layer may bind to some glue exposed on an edge of a tile of either a $\cgSE$ or a doubling row tile. We will denote the edge of a $\cgSE$ that abuts a tile location $i \in \{1,2,3,4,5,6\}$ by $e_i$.

Figure~\ref{fig:x2cgSE} shows the 3 tiles that make up a $\cgSE$ that can bind to two exposed $x2$ glues, while Figure~\ref{fig:xcgSE} shows the 3 tiles that make up a $\cgSE$ that can bind to two exposed $x$ glues.


Now we describe the various relevant tiles that may bind to a glue of a $\cgSE$ by location and describe the signals of the tiles of a $\cgSE$ that fire when a specific glue on an exterior edge of a $\cgSE$ binds to a complementary glue.


\begin{observation}\label{obs:pending-signals}
In each of the following cases, the tile $D$, $E$, and $F$ must be a tile belonging to $\alpha$ or a $frame$ layer. In either case, in order for the green $\cgSE$ to attach, it either attaches to $x$ glues exposed by $\alpha$, or a $q$ signal (in the $frame$ layer case) must have propagated through the tiles labeled $D$, $E$, and $F$.
\end{observation}


In each of the following we denote the green $\cgSE$ shown in Figure~\ref{fig:secgCases} by $CG$.

\begin{enumerate}[leftmargin=.3cm,itemindent=.3cm,labelwidth=\itemindent,labelsep=.3cm,align=left]
	\item \textbf{Location 1.}
	\begin{enumerate}[leftmargin=.3cm,itemindent=.3cm,labelwidth=\itemindent,labelsep=.3cm,align=left]
		\item Does not contain a tile\label{item:loc1notile}
			\begin{enumerate}
				\item[] By Observation~\ref{obs:pending-signals} and the fact that location 1 is empty, $D$ contains a tile that either exposes an $x$ or $x2$ glue or there is a pending signal to turn an $x2$ glue $\on$ on the east edge of $D$, or $D$ is empty. Therefore, in the case where $D$ is not empty, after $A$ binds to $D$ via the $x2$ glue $e_1$ exposes an $f2$ glue which initiates the growth of a $frame$ layer allowing for a single tile to attach at location 1 via cooperation of the $f2$ glue and the $x$ or $x2$ glue on $D$. On the other hand, if $D$ is empty, then a duple can attach via an $f2$ glue on the north edge of $A$ and an $x$ glue on the north edge of $E$.
			\end{enumerate}
		\item Contains a tile $t$ belonging to either $\alpha$ or the $frame$\label{item:loc1alpha}
			\begin{enumerate}
				\item[] After $CG$ binds, the east edges of $A$ and $B$ and the north edges of $B$ and $C$ expose $c$ glues. If an tile from the assembly surrounding $CG$ exposes an $x$ or $x2$ glue that allows for cooperative binding of either a checker tile or a checker duple (see Figure~\ref{fig:collision-detection-tiles}) via a $c$ glue and either an $x$ or $x2$ glue. When this $c$ glue binds, it sends a $q$ message through $A$, $B$, and $C$ that turn $x2$ glues $\on$ on the south edges of $B$ and $C$, and on the east edge of $A$. Moreover, this message turns $\off$ all of the $c$ glues for exposed by $CG$ and turns a $dr$ glue $\on$ on the east edge of $B$ that initiates the growth of a double row.
			\end{enumerate}
	\end{enumerate}	

	\item \textbf{Location 2.}
	\begin{enumerate}[leftmargin=.3cm,itemindent=.3cm,labelwidth=\itemindent,labelsep=.3cm,align=left]
		\item Contains a tile belonging to $\alpha$ or $frame$\label{item:loc2alpha}
			\begin{enumerate}
				\item[] First, just as in Case~\ref{item:loc1alpha}, after $CG$ binds, the east edges of $A$ and $B$ and the north edge of $B$ expose $c$ glues, and if an tile from the assembly surrounding $CG$ exposes an $x$ or $x2$ glue that allows for cooperative binding of either a checker tile or a checker duple via a $c$ glue and either an $x$ or $x2$ glue. This starts the propagation of a $q$ message and initiates growth of a double row.
				Secondly, the north edge of $C$ exposes a $c2$ glue. If location 6 is empty, and there is a $frame$ tile at location 2 that exposes a $c$ glue on its north edge, then a duple can bind via the $c2$ and $c$ glues. The binding of the $c2$ glue initiates the CCW propagation the $d$.
			\end{enumerate}
	\end{enumerate}	
	\item \textbf{Location 3.}
	\begin{enumerate}[leftmargin=.3cm,itemindent=.3cm,labelwidth=\itemindent,labelsep=.3cm,align=left]
		\item Contains a tile $t$ belonging to a $frame$ layer or double row\label{item:loc3frame}
			\begin{enumerate}
				\item[] In this case, if $t$ binds to the $x2$ glue of $C$, then this event signals a $cg$  glue on the north edge of $C$ to turn $\on$. Along with an $x2'$ glue, $t$'s south edge exposes a $cg'$ glue. When $cg$ and $cg'$ bind, this event initiates the propagation of a $q$ message through this frame layer through the frame layer that $t$ belongs to and through the frame layer that $CG$ belongs to.
			\end{enumerate}
	\end{enumerate}	


\end{enumerate}


To correctly send messages passed other concave corners we use relatively simpler corner gadgets. Figure~\ref{fig:cgNE} shows the $\cgNE$ tiles that form duples that allow a $frame$ layer to grow around a northeast corner. Note that once the duples form these tiles are capable of passing the $f$ signal CCW, and $q$ signals CCW and CW. Moreover, the $q$ signal turns all $c$ glues $\off$ and all $x2$ glues $\on$. To obtain the tile types for $\cgNW$ tiles rotate the $\cgNE$ tiles CCW and for $\cgSW$, rotate the $\cgNE$ tiles CCW twice.



==> non-rectangle-case-frame2.tex <==
\subsection{Handling collisions between $frame1$ and $frame2$}\label{sec:non-rect-f1-and-f2}

In the previous section we removed the restriction that $\alpha$ be a rectangle, and then discussed how $frame1$ grows in the absence of $frame2$.  This helped demonstrate many of the techniques needed to handle arbitrary series of both convex and concave corners around a perimeter, as a single-tile-wide path of tiles grows to completely cover it.  While $frame1$ is important for the fact that it forms a complete mold of $\alpha$ (to be used later), $frame2$ has a different function.  The purpose of $frame2$ is to grow a series of layers (each being a single-tile-wide path around the previous), as many as necessary, until exactly one layer of $frame2$ is precisely a rectangle.  This will eventually occur because each layer of $frame2$ is able to correctly determine if it is a rectangle and, if and only if not, initiate the growth of another layer, and each layer reduces the size of at least one concavity, thus bringing that layer closer to rectangular.  Let $frame2_i$ refer to the first layer of $frame2$ which is a rectangle around the outside of $\alpha$.  Since $frame2_i$ is the first rectangular layer, it is the first $frame2$ layer which is guaranteed to have exactly one $\cgSE$.  Once $frame2_i$ has completed, it is able to detect that it is a rectangle, and then from its single $\cgSE$ it initiates a message which propagates inward to $frame1$ in such a way that it arrives at exactly one tile of $frame1$, which can then be marked as a unique ``leader'' for $frame1$.  The importance of this in our shape replication constructions will be demonstrated later, but the techniques used to uniquely identify a single point on the perimeter of an arbitrary hole-free shape, a type of distributed leader election, seems to be of independent interest by itself.

In this section, we will discuss how the layers of $frame2$ grow, in addition to $frame1$, on non-rectangular $\alpha$ shapes.  However, in order to continue the process of adding functionality in a series of steps of increasing complexity, we will impose another restriction.  Namely, for now we will assume that each layer of $frame2$ completely finishes before any tile of the next layer attaches.  This will temporarily suspend our need to discuss how to handle collisions that may occur between tiles of different layers of $frame2$, but we will still need to handle collisions between $frame1$ and $frame2$ (since we won't assume that $frame1$ has completed), and also between different portions of the same layer of $frame2$.

Assuming that each $frame2$ layer fully completes before the next begins growth, we must cover the following:

MJP: some definitions:  The \emph{back} of a frame tile (either $frame1$ or $frame2$) is the side which served as input during its initial attachment with the glue $f'$ or $f2'$ (for a $frame1$ or $frame2$ tile, respectively).  The \emph{front} is the side opposite the back.  Similarly, the \emph{left} is the input side with the input glue $x'$ or $x2'$, and the \emph{right} side is the side opposite the left.  Note that we use these terms to talk about relative directions, and the cardinal directions N,E,S,W to talk about absolute directions, relative to individual tiles.

\begin{enumerate}
    \item There must always be a $frame1$ $\cgSE$ which is able to initiate a $frame2$ layer (i.e. there must be one which is not blocked from having a $\cgSE$ attach to its outside by some portion of $\alpha$ or $frame1$. Let $s \in EXT(\alpha)$ be the southernmost of the easternmost edges of the perimeter of $\alpha$.  Let $v$ be the vertex at the southern end of $s$.  By definition, there can be no tiles of $\alpha$ directly to the east, southeast, or south of the tile at $v$, and thus a $\cgSE$ of $frame1$ can attach.  After that attachment, the center tile of that $\cgSE$ becomes the southernmost of the easternmost tiles which compose the union of $\alpha$ and $frame1$.  By the same argument as for the $\cgSE$ of $frame1$, a $\cgSE$ of $frame2$ must be able to bind.\label{item:cgSE-can-always-bind}
    \item A $frame1$ $\cgSE$ can only allow a $frame2$ $\cgSE$ to attach to it if the entire portion of $frame1$ between it and the next $\cgSE$ in the CCW direction from it along $frame1$ is complete.  This is because the first $\cgSE$ will only activate the glues on its exterior which allow $frame2$ tiles to attach after it receives the $f_{done}$ message from the CW direction, which can only be initiated by the next CCW $\cgSE$.
    \item A $frame2$ layer grows similarly to $frame1$, starting from a $\cgSE$ and growing CCW one tile at a time (except for corner gadgets, which attach 2 or 3 tiles at a time). It passes an $f2$ message (rather than $f$) CCW as it grows.
    \item Upon reaching the first concavity (if any):
        \begin{enumerate}
        \item The last $frame2$ tile, denoted by $t_l$, of the current layer which can be placed without either the next being placed to its right or having no empty adjacent space (and we say that this last tile has hit a dead end), detects that it has hit a concavity when the $x2'$ glue on its front is able to bind to a tile in front of it.  At this point, it initiates an $r2$ message which passes backward through its $frame2$ layer until reaching the first corner (which must be convex since this is the first concavity).  As it passes through each tile along the way, it causes each to activate a glue on its right which can serve as input to an ``$r2r$'' tile (to be discussed).  Upon reaching the corner gadget at the first corner, that corner gadget activates a $cgr2$ glue which allows another corner gadget of a special $r2$ type to attach to its right. At this point, a ``doubling row'' for the current layer can form to the right of the first. Once it reaches the tile which detected the collision and initiated the $r2$ message, it then allows for the continuation of the growth of that layer of $frame2$ following the previous layer.  However, starting at the beginning of the doubling row and for the continuation of the path, rather than passing a $f2$ message, the path will now pass an $f2c$ message along to the next $\cgSE$.  See Figure~\ref{fig:concave-double-row} for a high-level depiction.

\begin{figure}[htp]
\centering
  \subfloat[][]{%
        \label{fig:concave-double-row}%
        \includegraphics[height=1.5in]{images/concave-double-row}
        }%
        \quad\quad
  \subfloat[][]{%
        \label{fig:frame2-concave-collisions}%
        \includegraphics[height=1.7in]{images/frame2-concave-collisions}
        }%
  \caption{An example showing the growth of a portion of a $frame2$ layer when encountering the first concave corner. (Left) A small portion of an inner frame layer (grey) with a $frame2$ layer growing on its exterior.  The yellow portions show the growth of the new layer, with the main messages shown (and the gold representing a new 2-tile $\cgSE$ which is functionally the same as the other but passes an $f2c$ message instead of $f2$).  While growing from a $\cgSE$ of a $frame2$ layer, a path of tiles initially passes forward an $f2$ message.  However, when that path reaches the first concave corner, it passes an $r2$ message backward until it reaches the first corner gadget, along the way activating glues which allow special ``doubling row'' tiles to attach to their right sides.  The corner gadget activates glues that allow the new corner gadget and row of tiles to grow (while passing an $f2c$ signal) along the previous row.  As soon as this new row is blocked from forward growth, it continues growth of the $frame2$ layer in the regular way, but now passing an $f2c$ message to indicate that a concave corner has been encountered.  Note that if there is not enough room within the concavity for a second row to form, the same methods used to pass other signals out of a concavity are used to ensure that the frame can continue growth, passing the $f2c$ message along. (Right) Beginning of an image to show how $frame2$ collisions are ignored in the first tile of a concavity. Needs more work.}
  \label{fig:frame2-concave}

\end{figure}

        \item The first row into a concavity will collide with the previous layer (on which it is growing), but that previous layer must ``ignore'' the collision and not attempt to pass the $f2$ signal, as depicted in Figure~\ref{fig:frame2-concave-collisions}.  This prevents an $f2$ signal from attempting to propagate back through the tiles of a previous layer effectively propagate this $f2$ signal in the CW direction relative to the previous frame, even though it this $f2$ signal could propagate in the CCW direction (For example, by adding more tiles to this layer of $frame2$ as in Figure~\ref{fig:frame2-concave-collisions}.) This is accomplished as follows. Once $t_l$'s $x2'$ glue along its front, instead of triggering an $f2$ glue on its right, $t_l$ triggers an $f2_{ab}$ where $a$ and $b$ are distinct elements of $\{n,s,e,w\}$ and depend on which two edges of $t_l$ are its left and front edges respectively. (For example, in Figure~\ref{fig:frame2-concave-collisions}, the glue that is triggered to turn $\on$ is the $f2_{wn}$ glue on the eastern edge of $t_l$.) Then, we create a special tile type that can bind to an $x2$ and $f_{ab}$. This tile behaves exactly like its counterpart that binds to an $x2$ and $f2$ glue (See Figure~\ref{fig:post-collision-handling}.), except that unlike $f2'$, $f2_{ab}'$ does not trigger an $f2'$ glue on the right edge to turn $\on$. [JGH: figure of this special tile?]
        \item If there is no gap to the right of (some of) the tiles which propagate the $r2$ message (including the corner gadget), the returning doubling row grows as far as possible and then, following standard procedure, rotates the path and continues to grow and/or pass the $f2c$ signal.
        \end{enumerate}

    \item When an $f2$ or $f2c$ message reaches the next $\cgSE$, that corner gadget initiates the backward propagation of an $f2_{done}$ or $f2c_{done}$ message, respectively, and activates glues on its north side which can receive either signal.  This backward propagation is done in the same way as described for messages in $frame1$ (Section~\ref{sec:signal-following}).

    \item When an $f2$ or $f2c$ message is received by the north side of a $frame2$ $\cgSE$, that $\cgSE$ now has information indicating whether there are any concave corners between it and the next $\cgSE$ in the CCW direction and also between it and the next $\cgSE$ in the CW direction.
        \begin{enumerate}
        \item If either message is $f2c$, then this $\cgSE$, call it $C$, ``knows'' that this layer is not a rectangle and it will activate glues which allow a new $frame2$ layer to begin by the attachment of a $\cgSE$ to its outside. To activate these glues, a $nr$ message originating from $C$ follows the $f2$ signal in order. When the $nr$ message is passed to the southeast tile of a $\cgSE$, signals trigger glues to turn $\on$, exposing $x2$ glues that could allow for the a $\cgSE$ of a new $frame2$ layer to bind. [JGH: don't forget about the case where a special corner tile that handles the weird staircase cases is at the southeast corner]
        \item If both messages are $f2$, then the $\cgSE$ ``assumes'' that this layer is a rectangle.  It therefore initiates a CCW message to cause the detachment of the portion of that $frame2$ layer between that $\cgSE$ and the next which is immediately CCW of it on that $frame2$ layer. As stated in Case~\ref{item:f2-arrives} of Section~\ref{sec:rectangles}, it also activates the primer on the layer inside it.
        \end{enumerate}

    \item As in the rectangular case, (Case~\ref{item:f2-arrives} of Section~\ref{sec:rectangles}), if a completed $frame2$ layer is a rectangle, it will be able to detach.  Note that if the layer has a doubling row it is not considered rectangular since an $f2c$ signal fires when a double row attaches to a frame.



\begin{figure}[htp]
\centering
    \includegraphics[width=2.5in]{images/frame-cant-detach}
    \caption{An example input assembly $\alpha$ with enough convex corners to result in a $\cgSE$ to mistakenly interpret its location as being the SE corner of a rectangle.  The grey portion represents $\alpha$ as well as the $frame_1$ which initially grew around it.  The yellow, blue, red, and green represent a $frame_2$, where the red are $\cgSE$ which receive signals telling them they are not SE corners of a rectangle (thus causing them to initiate growth of another $frame_2$ layer), and the green represents a $\cgSE$ which receives signals causing it to behave like it is the SE corner of a rectangle.  The result is for it to send a ``detach'' message CCW, which is depicted by the blue section.  This signal terminates at the next $\cgSE$ in the CCW direction, and therefore the red and yellow portions ensure that the frame remains attached.}\label{fig:frame-cant-detach}
\end{figure}

    \item If a completed $frame2$ layer is not a rectangle, then
        \begin{enumerate}
        \item It will not be able to detach: (See Figure~\ref{fig:frame-cant-detach} for an example of a frame layer which partially attempts to detach.)

            \begin{enumerate}
            \item The initial growth of the layer ensures that every individual tile and gadget attaches to the ring inside it with at least one glue (more for corners of concavities).

            \item The only time tiles deactivate glues which allow them to detach from the frame inside of them is when they receive a CCW moving signal which originates from a $\cgSE$ which has detected that the four corners most immediately CCW of it are all convex, as are the four corners most immediately CW of it. Initially, the CCW moving signal will begins by deactivating the glues on the western edge of the northern most tile of a $\cgSE$. Then, this signal deactivates the glues on the western edge of each consecutive tile following the $f2$ message. When the deactivation signal reaches the next $\cgSE$, it triggers the deactivation of the glues on the northern edge of the the westernmost tile of this $\cgSE$.
			\item The $\cgSE$, $CG_0$, that starts the deactivation signal is bound to the previously added frame by at least one strength-1 glue. In fact, either its westernmost tile is bound to the previous frame or its westernmost tile is bound to a portion of the current $frame2$ layer, and this portion of the frame layer must contain at least all of the tiles of the current frame up to the next $\cgSE$, $CG_1$, in the CW direction. Then, the next $\cgSE$ in the CW direction must also be bound to $frame1$ or the previous frame layer (in which case, $CG_0$ is bound to $frame1$ or the previous frame layer by at least one strength-1 glue) or must be bound to a portion of the current $frame2$ layer, and \emph{this} portion of the frame layer must contain at least all of the tiles of the current frame up to the next $\cgSE$, $CG_2$, in the CW direction. Since we are in the case where the completed $frame2$ layer is not rectangular, if we continue with this argument, eventually, we arrive at a $\cgSE$, $C_n$, that must be bound to $frame1$ or the previous frame layer. This follows from the fact that some $C_n$ must receive an $f2c$ signal instead of an $f2$ signal, and therefore, will not deactivate any of its glues that bind it to $frame1$ or the previous frame layer.
			\item The next $\cgSE$ after the $\cgSE$ that starts the deactivation signal in the CCW direction is bound to the previously added frame by at least one strength-1 glue. This follows by a similar argument used in the previous case. [JGH: does this take care of the next item]
            \item For any complete frame [MJP: CONTINUE HERE, explain why incomplete frames aren't a problem!] which is not a rectangle, there exists a $\cgSE$ such that one of the three nearest corners in either the CCW or CW direction which is a concave corner. [MJP: Prove this]
            \item Therefore, the tiles of that $\cgSE$ will not detach from the inner frame, and since all tiles of the frame are $\tau=2$ stably bound together (via at least $f2$ or $f2c$ and $f2_{done}$ or $f2c_{done}$ glues), the entire frame is prevented from detaching
            \end{enumerate}

        \item and it will initiate the growth of another $frame2$ layer:

            \begin{enumerate}
            \item A rectangle is the only shape whose perimeter has exactly 4 sides and exactly 4 convex corners.  (The perimeters of all other shapes have $> 4$ convex corners.)  This follows directly from the definition of a shape as a finite, connected subset of $\Z^2$.

            \item Any shape which is not a rectangle has at least 1 concave corner.  This is because a rectangle's perimeter has the minimum number of sides for a shape, as well as 4 convex corners, and adding any side requires the addition of a concave corner.

			\item On the perimeter of a non-rectangle, at least one $\secon$, which we will denote as $\secon'$, must be within $3$ vertices in the CCW direction of a concave corner.
			
            \item The $\cgSE$ at $\secon'$ will receive a $f2c$ signal [JGH: or we have a staircase case], which will cause it to pass an $nr$ message that follows $f2$ in order. When the $nr$ message is passed to the southeast tile of a $\cgSE$ [JGH: or we have a staircase case], signals trigger glues to turn $\on$, exposing $x2$ glues that could allow for the a $\cgSE$ of a new $frame2$ layer to bind. This ensures that each $\secon$ exposes two $x2$ glues. One on a south edge and one on an east edge.

            \item On the perimeter of a non-rectangle, as seen in Case~\ref{item:cgSE-can-always-bind}, at least one $\secon$ will have south and east edges each of which exposes an $x2$ glue such that a $\cgSE$ can attach via these exposed glues and initiate the growth of another $frame2$ layer.

            \end{enumerate}
        \end{enumerate}

    \item A $frame2$ layer may not be able to grow into an concavity because it may have already been filled by $frame1$ and possibly $frame2$ layers. In that case, the $frame2$ layer simply grows over the frame layers which were able to grow into it (or those which have already grown outside of those).

    \item $frame2$ layers handle collisions with layers of $frame2$, $frame1$, and $\alpha$. [MJP: much discussion here!]
        \begin{enumerate}

		\item To handle collisions between a $frame2$ layer and itself, we enhance the tiles of $T_{f2}$ in exactly the same way that we enhanced the tiles of $T_{f1}$ described in Section~\ref{sec:frame1-collision}, except there, the $f$ message is being passed, and in the case of $frame2$, the $f2$ message is being passed.
		
		\item Collisions between a $frame2$ layer and $frame1$, are handled as follows.

		\begin{enumerate}
			\item When a tile of $frame2$ detects a collision with $frame1$, with the exception of one special case, the tiles of $frame1$ simply ``ignores'' the $f2$ message. [JGH: we need to show that this can only occur in ``frame holes''] In other words, the tiles of $frame1$ do expose $f2$ glues, with the exception that they do expose $f2$ glues in cases similar to the case depicted in Figure~\ref{fig:frame2-concave-collisions}. In Figure~\ref{fig:frame2-concave-collisions}, when the orange frame is $frame1$ (and passing an $f$ message instead of an $f2$ message) and the yellow frame $frame2$ detects a collision with $frame1$, the tile, $t$, that is one tile to the right of the concave corner tile exposes an $f2$ glue that triggers an $r2$ glue to be exposed on the south edge of $t$. This will ensure that the $\frametwo{1}$ assembles a ``double row'' and then continues to propagate the $f2$ message CCW either by continuing to grow or by propagating this message through collisions with $frame2$ tiles.
        \item Explain how collisions are handled by cascading signals using the technique of Figure~\ref{fig:signal-ordering} and the necessary number will be propagated. [JGH: I think we can refer to the next section for this]			
			\item When $frame1$ detects a collision with $frame2$, $frame2$ propagates the $f$ message exactly like $frame1$ tiles would. We accomplish this by further enhancing the tiles of $T_{f2}$, analogous to the enhancements described in the case of collisions between $frame1$ and itself in  Section~\ref{sec:frame1-collision}, so that they can pass the $f$ message CCW. In particular, a tile of $frame2$ is capable of passing an $f$ message as well as an $f2$ message CCW and CW. This will ensure that an $f$ message can always propagate from a $\cgSE$ to the next $\cgSE$ in the CCW direction. [JGH: this may be too terse and imprecise]
		\end{enumerate}				

        \item Explain how collisions are handled by cascading signals using the technique of Figure~\ref{fig:signal-ordering} and the necessary number will be propagated. [JGH: I think we can refer to the next section for this]

        \item To do this, each $frame2$ layer is able to pass a single $f1$ signal and also a single $f2$ in each direction
        \item Also, $frame2$ tiles which have received an $f1$ signal can ``behave like $frame1$ tiles. [MJP: need more details!]
        \item To handle a corner case, $frame1$ signals must be able to ``bounce back'' $f2$ signals on their input sides (after initially binding using an $f$ signal).
        \item $frame_2$ signals around the outside of the shape cannot be lost (although some inside enclosed concavities may).  For each enclosed concavity, as many $frame_2$ signals which enter eventually exit.  [Prove this]
        \end{enumerate}
    \item  Eventually, after a sufficient number of $frame2$ layers have assembled, the concavity will be filled in, and thus eventually all will. Therefore, as $frame2$ assembles layer by layer, eventually some $frame2$ layer will be rectangular and thus able to detach.

    \item If a frame detaches, it must be a rectangle and have marked exactly one inner tile of the $frame2$ row immediately inside of it, which now becomes the \emph{marked} tile.

    \item A signal from the single marked tile on the $frame_2$ ring which was immediately inside the first rectangle layer begins inward propagation until it reaches the easternmost tile of the southern most tiles of $frame_1$, call this tile $t$, at which point it begins a $done$ signal that moves CCW around $frame_1$. The signal that propagates inward until it reaches $t$ is described in Figure~\ref{fig:marking-frame1}.

    \item When that $done$ message returns to the $frame_1$ tile from which it initiated, it initiates $kill$ message which propagates through the entire $frame_1$.  That $kill$ message causes every connection to $\alpha$ via $x$ glues to break by deactivating the connected glues.

    \item When the $kill$ signal returns to the tile which initiated it, the final glues holding $frame_1$ to $\alpha$ deactivate, allowing an assembly consisting of all $frame_1$ and $frame_2$ tiles (except the outer ring which already detached) to separate from $\alpha$. We call this the \emph{frame} for $\alpha$.
\end{enumerate}


\subsection{Handling collisions between different $frame2$ layers}

In Section~\ref{sec:non-rect-f1-and-f2}, we discussed the methods for handling collisions between $frame1$ and $frame2$, but we temporarily assumed that different layers of $frame2$ do not collide with each other (i.e. each fully completes before any growth of the next).  In this subsection, we remove that assumption and discuss how collisions of different layers of $frame2$ may occur and how they are handled by the construction.

What we need to prove to guarantee the correctness of the construction is that regardless of how portions of $frame2$ layers collide with other portions of $frame2$ layers, the following properties hold:

\begin{enumerate}
    \item A sufficient number of layers will form for one of them to be rectangular
        \begin{enumerate}
            \item There is always at least one $\cgSE$, say $c$, such that there is space available for another $\cgSE$ to attach to the southeast corner of $c$. (This property holds for any shape, as has previously been shown.)  Assuming that $c$ receives an $f2c_{done}$ signal, it will activate the glues necessary to allow the next $\cgSE$ to bind to it, as well as a signal which will propagate completely around that layer activating the $x2$ .
            \item A CCW growing path of $frame2$ tiles will be initiated from that (and possibly other) $\cgSE$'s.
            \item These paths will be able to grow around convex corners via the typical corner gadgets.
            \item When convex corners are encountered, layers will be able to grow in and out, and one of the following will hold:
                \begin{enumerate}
                    \item the number of rows in equals the number out:  in this case the concavity is filled in
                    \item the number of rows in is less than the number out:  in this case, rows will continue to grow from behind and collide with the set that grows out until they are of even height (I think this is easy enough to argue)
                    \item the number of rows in is greater than the number out:  in this case, the ``new tile'' (described below) allows new segments of $frame2$ to begin immediately beyond the concavity for each extra row in, eventually smoothing it out
                \end{enumerate}
            \item Since It is obvious that a $frame2$ layer can continue growth along a straight edge [MJP: have to gurant
        \end{enumerate}
    \item The first rectangular layer will recognize that it is rectangular, halt the growth of new layers, and initiate the inward traveling ``marking'' signal
        \begin{enumerate}
            \item if a rectangular layer can grow, a $\cgSE$ which can initiate it must be able to attach and begin the growth of that layer
            \item only the ``standard'' tiles which can grow around a rectangle will be able to attach
            \item the layer will be able to grow completely around because nothing can block it
            \item the layer can receive no signals from layers within, because it binds on the inside only to $x2$ glues, and no side of a tile which binds to an $x2$ glue can receive a signal
            \item therefore, the $f2$ and $f2_{done}$ signals will be sufficient for the layer to determine its a rectangle, prevent it from allowing another $\cgSE$ gadget from attaching, and initiate the inward ``marking'' signal
        \end{enumerate}
\end{enumerate}

The new tile is like a regular $frame2$ tile for a straight segment except that one input is $x2$ and the other is a special glue $f2x$.  The glue $f2x$ is exposed on the right side of a $frame2$ tile whose successor in the path determined that adjacent to its right side is a corner gadget, and sent a signal back to its predecessor directing it to activate an $f2x$ glue on its right side.

Boo ya.



\begin{enumerate}
    \item If an $f2$ signal is being passed backward through a $frame2$ layer, it continues to be passed backward until there it can be output to a location which will allow for the placement of a new $frame2$ tile and the continuation of growth of a $frame2$ layer.  See Figure~\ref{frame2-frame2-collision} for an example showing a collision between portions of $frame2$ layers growing in opposite directions (at the blue and yellow collision near the center).  In this case, the $f2$ signal which initiated in the blue segment passes backward through the entire series of yellow portions.  [MJP: continue this explanation]
    \item $frame2$ layers may ``die'' within concavities, but as many $f2$ signals enter while passing forward through a $frame2$ layer will also eventually exit (although the path taken may not...  This can also be seen in Figure~\ref{frame2-frame2-collision} as the order of growth shown results in two $f2$ signals... [MJP: maybe its better to talk about the number of layers which can grow before and after!]
    \item The necessary number of $frame2$ layers to eventually form an external rectangular level will form since ``external'' $frame2$ layers can always complete and become closer to rectangular
\end{enumerate}


Figure~\ref{fig:signal-ordering} shows how to augment a frame tile so that it can receive a message in each of its output (i.e. front and right) sides, in any order, and always output that message first to its back side, then its left side.
\begin{figure}[htp]
\centering
  \subfloat[][Original version where a ``message'' in the form of the signal $sig$ can be received from the north and east, and propagated to the south and west]{%
        \label{fig:signal-down-and-left}%
        \makebox[2.0in]{\includegraphics[width=1.5in]{images/signal-down-and-left}}
        }%
        \quad\quad\quad
  \subfloat[][Enhanced version where $sig$, now represented as the union of $sig_1$ and $sig_2$, is guaranteed to be passed south first, and if later received from a second direction, then it's passed west.]{%
        \label{fig:signal-down-first-left-second}%
        \makebox[2.0in]{\includegraphics[width=1.5in]{images/signal-down-first-left-second}}
        }%
  \caption{An example of how to modify signals to propagate a message down the first time it is received, and to the left the second time it is received.}
  \label{fig:signal-ordering}
\end{figure}


\begin{figure}[htp]
\centering
    \includegraphics[width=2.5in]{images/frame2-frame2-collision}
    \caption{MJP: Crazy case where $f2$ signal bounces backward like a mofo.}\label{fig:frame2-frame2-collision}
\end{figure}




==> non-rectangle-case.tex <==
\subsection{Framing non-rectangles}\label{sec:non-rectangles}

We now turn our attention to the more complex case of non-rectangular input assemblies. We will first describe how $frame1$ assembles under the assumption that $frame1$ completes assembly before any $frame2$ tiles bind. As $frame1$ assembles, we show how we modify the tiles of $T_{f1}$ in order to introduce signal based gadgets that handle the many special cases that arise. Now, let $\alpha$ be a non-rectangular input assembly. $frame1$ assembles around $\alpha$ as follows.

\begin{enumerate}
	\item As in the case where $\alpha$ is rectangular, the first tile attachment to $\alpha$ must consist of a 3-tile $\cgSE$ attaching to a single $\secon$ corner of $\alpha$. Since $\alpha$ is non-rectangular, it may have multiple $\secon$ corners, each of which allows for the attachment of a single 3-tile $\cgSE$. (The red tiles in Figure~\ref{fig:frame1-nonrectangle} depict $\cgSE$'s.)
	\item From a $\cgSE$, a single-tile-wide path grows CCW with each tile binding to the $x$ glue on $\alpha$ and the output $f$ glue of the immediately preceding tile.  In this way, we say the the $f$ message is passed CCW through $frame1$.  (See Figure~\ref{fig:frame1-nonrectangle}.)

\begin{figure}[htp]
\centering
    \includegraphics[width=2in]{images/frame1-nonrectangle}
    \caption{An example showing how a frame growing around a non-rectangular shape $\alpha$ correctly passes the $f$ message.}\label{fig:frame1-nonrectangle}
\end{figure}
	
    \item If a tile of $frame1$ arrives at a location adjacent to the:
        \begin{enumerate}
        \item western edge of a $\cgSE$, the $f$ message is passed to the center tile of the $\cgSE$, which then initiates the propagation of an $f_{done}$ message back through $frame1$ that follows the $f$ message in the opposite direction of the $f$ message. That is, if the $f$ message passes through a sequences of tiles $\langle\T_i\rangle_{i=0}^n$ (not necessarily distinct) in order, then the $f_{done}$ message is passed through the sequence $\langle\T_{n-i}\rangle_{i=0}^n$ in order. In Section~\ref{sec:signal-following}, we show how to enhance (add signal glues and modify existing signal glues) the tiles of $T_{f1}$ so that each tile used to pass the $f$ message ``records'' (using signal glues) the direction that the $d_{done}$ message should be passed in order to follow the $f$ message in reverse. The $\cgSE$ also activates a glue on its northern side to receive such a signal once it has completed its path around $frame1$. \label{item:CCW-growth}
        \item souther edge of a $\cgSE$, [MJP: describe this new f'd up case]
        \end{enumerate}
    \item If a tile $t$ of $frame1$ arrives at a location where the left most tile of a 3-tile $\cgSE$ could have attached (thus preventing a 3-tile $\cgSE$ from binding), then growth of this portion of the path pauses until a 2-tile $\cgSE$ binds via the $f'$ and $x'$ glues of the 2-tile $\cgSE$ and the $f$ glue of $t$ and the $x$ glue of the tile of $\alpha$ directly north of $t$. When the 2-tile $\cgSE$ binds, we are essentially back in Step~\ref{item:CCW-growth} where the $f_{done}$ message is initiated.
    \item If a north-growing tile $t$ of $frame1$ (i.e. one that grows along an eastern edge of $\alpha$) arrives at a location adjacent to the southern edge (the western, eastern and northern edge case is similar up to rotation) of a tile in $T_{f1}$, we say that $frame1$ \emph{collides} with itself. (See location $L1$ in Figure~\ref{fig:frame1-self-collisionA}.) In this case, we continue to pass the $f$ message CCW through the portion of the frame that was collides with. In order to accomplish this we must once again enhance the tiles of $T_{f1}$ so that each tile can \emph{detect collisions} with tiles of $frame1$, and so that each tile can propagate the $f$ message once CCW and once CW. (See Figure~\ref{fig:frame1-self-collisionB}.) For a description of these enhancements, see Section~\ref{sec:frame1-collision}.
    \item If a tile of $frame1$ arrives at a location adjacent to the southern edge (the western, eastern and northern edge case is similar up to rotation) of a tile of $\alpha$, we say that $frame1$ \emph{collides} with $\alpha$. (See highlighted tile location labeled $A$ in Figure~\ref{fig:frame1-single-tile-wide-concavity}.) In this case, we continue to pass the $f$ message CCW. In order to accomplish this we must once again enhance the tiles of $T_{f1}$ so that each tile can detect collisions with tiles of $\alpha$, and so that each tile can propagate the one copy of the $f$ message CCW, and one more copy CW. These tile enhancements ensure that every $f$ message initiated from some $\cgSE$ is guaranteed to eventually arrive at the next $\cgSE$ in the CCW direction. For a description of these enhancements, see Section~\ref{sec:frame1-collision}.  Moreover, these enhanced tiles are capable of ``filling'' single-tile-wide concavities as depicted in Figure~\ref{fig:frame1-single-tile-wide-concavity}. 	
	
\begin{figure}[htp]
\centering
  \subfloat[][$frame1$ originates from a $\cgSE$, enters a single tile wide concavity.]{%
        \label{fig:frame1-self-collisionA}%
        \makebox[2.7in][c]{\includegraphics[width=1.5in]{images/frame1-self-collisionA}}
        }%
        \quad\quad
  \subfloat[][We allow the tiles of $frame1$ to pass one $f$ message in each direction so that when there is a collision between $frame1$ and itself, the $f$ message can still be passed.]{%
        \label{fig:frame1-self-collisionB}%
        \makebox[2.7in][c]{\includegraphics[width=1.7in]{images/frame1-self-collisionB}}
        }%
  \caption{How to handle collisions between $frame1$ and itself.}
  \label{fig:frame1-self-collision}
\end{figure}


\begin{figure}[htp]
\centering
    \includegraphics[width=1.5in]{images/frame1-single-tile-wide-concavity}
    \caption{An example showing how a frame growing around a non-rectangular shape $\alpha$ correctly passes the $f$ message. This is the basic technique used to correctly detect when a frame grows into a concavity and route the $f$ message in a CW direction, $90$ degrees at a time, until it can again propagate.  This may result in a $90$ degree turn creating a new path of tiles, or a $180$ degree turn passing the message back down the currently existing path (in the reverse of the direction it previously moved), until it can again continue new growth.}\label{fig:frame1-single-tile-wide-concavity}
\end{figure}	
				
    \item Once the $f_{done}$ message arrives at the north side of a $\cgSE$ gadget, that gadget then turns on the two glues necessary to allow for the attachment of a $\cgSE$ gadget for the first $frame_2$ layer (which will eventually consist of a ring of tiles around $frame_1$).  In this way, and because the single-tile-wide path of tiles referred to as $frame_2$ will grow CCW in a way similar to $frame_1$, it is ensured that the portion of $frame_1$ between $\cgSE$ gadgets (if there are more than one, otherwise it's just a path between two sides of the same $\cgSE$ gadget) must be completed before any portion of the $frame_2$ layer can begin growth along the outside of that portion of $frame_1$. Furthermore, just as shown for $\cgSE$'s of $frame1$, there must always be at least one $\cgSE$ to which another can attach.
	
	
	
\end{enumerate}



\subsubsection{Detecting $frame1$ collisions with $\alpha$ and $frame1$}\label{sec:frame1-collision}

In this section, we describe how we can ``enhance'' the tiles of $T_{f1}$ so that they are capable of passing the $f$ message even in the cases where a collision with $frame1$ or a collision with $\alpha$ occur. These enhancements will be signal glue additions and modifications to the tiles of $T_{f1}$. For an overview, see Figure~\ref{fig:collision-handling}.  Essentially, in order to detect a collision with $\alpha$ on side $s$, a glue of type $x'$ is activated on side $s$ since that will be able to bind with the exposed $x$ glue of the tile in $\alpha$, and similarly in order to detect a collision with a $frame1$ tile a glue of type $f'$ is activated since a collision with a $frame1$ tile occurs when a side outputting $f$ of one tile is incident with a non-input side of another.

\begin{figure}[htp]
\centering
  \subfloat[][A basic frame building tile which allows for northward growth via the $f$ message.]{%
        \label{fig:pre-collision-handling}%
        \makebox[2.7in][c]{\includegraphics[width=1.5in]{images/pre-collision-handling}}
        }%
        \quad\quad\quad
  \subfloat[][The same tile enhanced to detect collisions with walls due to concavities and also with other frame rows.  The additional signals allow it to turn the corners of concavities and to correctly pass the $f$ message after any collision.]{%
        \label{fig:post-collision-handling}%
        \makebox[2.7in][c]{\includegraphics[width=1.5in]{images/post-collision-handling}}
        }%
  \caption{How to handle collisions with walls (due to concavities) and with other frame rows.}
  \label{fig:collision-handling}
\end{figure}

Defining tiles of $T_{f1}$ that use the scheme in Figure~\ref{fig:post-collision-handling} gives tiles capable of placing tiles of a frame around $\alpha$ in a CCW direction. For example, consider the tiles of a frame that is growing northward. The southward, eastward and westward cases are handled the same way upto rotation. Let the last tile of this northward growth be called $F$. There are 6 cases to consider where one or more collisions occur.

\begin{enumerate}
	\item There is a tile $T_n$ directly to the north of $F$ that is a tile of $\alpha$, and
		\begin{enumerate}
			\item There is a tile $T_e$ directly to the east of $F$ that is a tile of $\alpha$.\label{item:collision-case1a}
			\item There is a tile $T_e$ directly to the east of $F$ that is not a tile of $\alpha$.\label{item:collision-case1b}
			\item There is not a tile directly to the east of $F$.\label{item:collision-case1c}
		\end{enumerate}
	\item There is a tile $T_n$ directly to the north of $F$ that is not a tile of $\alpha$, and
		\begin{enumerate}
			\item There is a tile $T_e$ directly to the east of $F$, that is a tile of $\alpha$.\label{item:collision-case2a}
			\item There is a tile $T_e$ directly to the east of $F$, that is not a tile of $\alpha$.\label{item:collision-case2b}
			\item There is not a tile directly to the east of $F$.\label{item:collision-case2c}
		\end{enumerate}
\end{enumerate}
 
In Case~\ref{item:collision-case1a}, the tile $T_n$ prevents northward growth of the frame. From Figure~\ref{fig:collision-handling}, we can see that $F$ will attempt to pass the $f$ message to the east. However, any eastward growth of the frame will be prevented by the tile $T_e$. Since $T_e$ exposes an $x$ glue, $F$ will pass the $f$ message to the south. This is shown schematically in the highlighted region labeled $A$ in Figure~\ref{fig:frame1-single-tile-wide-concavity}.

In Case~\ref{item:collision-case1b}, $T_e$ must be a tile that belongs to another portion of $frame1$, and it will expose an $f'$ glue to allow for the $f$ message to be passed to the east. Also, $T_e$ will expose an $f$ glue which must be propagated to the south of $F$. For this reason, $F$ exposes an $f'$ glue which will pass the $f$ message that $T_e$ is propagating to the south. This is shown schematically in the highlighted region labeled $B$ in Figure~\ref{fig:frame1-single-tile-wide-concavity}.

In Case~\ref{item:collision-case1c}, $F$ will expose an $f$ glue that will allow for $frame_1$ to continue growth CCW. If some frame places a glue directly to the east of $F$, then we are back in Case~\ref{item:collision-case1b}.

In Case~\ref{item:collision-case2a}, the tile $T_n$ prevents northward growth of the frame.  Since $T_n$ is a copy of a tile in $T_{f1}$, it will allow for an $f$ message to be passed to it. Therefore, $F$ will pass an $f$ message to the north. Now notice that the north edge of $F$ exposes a glue $f'$. Since $T_n$ is not a tile of $\alpha$, $T_n$ must be a copy of a tile in $T_{f1}$ and the glue exposed on the north edge of $F$ will allow $T_n$ to pass an $f$ message to $F$ should the CCW propagation of the $f$ message require $T_n$ to pass the $f$ message to the south. This is depicted in the highlighted region labeled A in Figure~\ref{fig:collision-handling-2ac}.  Then, since $T_e$ is a tile of $\alpha$, it exposes an $x$ glue so that when the $x'$ glue on the east edge of $F$ binds to this glue, will pass the $f$ message to the south.

\begin{figure}[htp]
\centering
    \includegraphics[scale=0.03]{images/collision-handling-2ac}
    \caption{An example of $frame1$ collision Cases~\ref{item:collision-case2a} and~\ref{item:collision-case2c}.}\label{fig:collision-handling-2ac}
\end{figure}	

In Case~\ref{item:collision-case2b} and Case~\ref{item:collision-case2c}, like in the previous case, $F$ will pass an $f$ message to the north. However, in Case~\ref{item:collision-case2b}, if $T_n$ passes an $f$ message to $F$, since $T_e$ is a copy of a tile in $T_{f1}$, it will allow $T_e$ to propagate the $f$ message to the east. This is shown in the region labeled B in Figure~\ref{fig:collision-handling-2b}. In Case~\ref{item:collision-case2c}, $F$ will expose an $f$ signal that will allow for $frame1$ to continue CCW growth. This is shown in the region labeled C in Figure~\ref{fig:collision-handling-2ac}.

\begin{figure}[htp]
\centering
    \includegraphics[scale=0.03]{images/collision-handling-2b}
    \caption{An example of $frame1$ collision Case~\ref{item:collision-case2b}.}\label{fig:collision-handling-2b}
\end{figure}	

Note that the signal tiles presented in Figure~\ref{fig:collision-handling} are capable of completely ``filling'' a single-tile-wide concavity. Figure~\ref{fig:signals-through-concavities} gives an example of this.

\begin{figure}[htp]
\centering
    \includegraphics[width=3in]{images/signals-through-concavities}
    \caption{An example showing how a frame growing through a concavity correctly passes the $f$ message (using the signal patterns shown in Figure~\ref{fig:post-collision-handling}) and continues growth through the entire concavity.  This shows just a small portion of a frame, with the growth beginning in the south.}\label{fig:signals-through-concavities}
\end{figure}		

\input{signal-following}

\begin{figure}[htp]
\centering
  \subfloat[][An example showing the outermost two $frame_2$ layers, where the outermost is the first which is a rectangle.  Thus, the $\cgSE$ gadget shown in green will initiate signals that cause $frame_2$'s dissociation, etc.]{%
        \label{fig:frame-can-detach}%
        \includegraphics[width=3.0in]{images/frame-can-detach}
        }%
        \quad\quad
  \subfloat[][A zoomed in view of a few of the tiles represented in Figure~\ref{fig:frame-can-detach}.  This demonstrates how the arrival of the appropriate message (here represented as simply as \emph{rectangle}) in the $\cgSE$ of a rectangular $frame_2$ activates the $p'$ glue which binds to the $frame_2$ inside it, thus \emph{priming} it.  This binding then initiates the \emph{detach} signal in the outer $frame_2$ which causes that entire frame to detach from that inside it.  It also causes the inner $frame_2$ to activate a $p_2$ glue which, once the outer ring dissociates (and only once that happens), is able to bind with a tile of the grey type, and this binding initiates the inward propagation of the $kf_1$ message which eventually reaches the $frame_1$.]{%
        \label{fig:frame-can-detach-primed}%
        \includegraphics[width=3.0in]{images/frame-can-detach-primed}
        }%
  \caption{An example showing how a detaching $frame_2$ can initiate the ``priming'' of the frame immediately inside it, causing the inward propagation of the signal which eventually reaches $frame_1$, uniquely marks one position of it, and causes the entire mold to detach from $\alpha$.  It is important to note that whenever a $frame_2$ layer is not a rectangle, even if some of the $\cgSE$ gadgets of that frame receive messages indicating that they are on a rectangle and initiate detachment messages, because of the fact that there must be at least on $\cgSE$ gadget of that frame which doesn't receive the \emph{rectangle} message, at least the tiles of that gadget will remain attached to the inner frame and prevent the entire outer frame from detaching.  Because of this, even though some of the $\cgSE$ of the inner frame may be primed, those primed tiles will be blocked from binding with $p_2$ tiles by the still attached outer frame, and thus won't initiate the (possibly multiple) messages which would attempt (and fail) to uniquely mark one position of $frame_1$.}
  \label{fig:frame-priming}
\end{figure}

\input{non-rectangle-case-frame2} 

==> replication.tex <==
\section{Replication}

[I need to think more about the distinctions between ``replication'' and ``self-replication'' and determine which results can be put into which category.  ]

In this section, we provide constructions in the STAM which are capable of replicating assemblies.  In the interest of simulating biological behavior, some of our results strive to be self-replicating, i.e. individual assemblies initiate the process by which they replicate, and identical copies of those assemblies are created, tile for tile.  For these, the self-replication is unbounded, theoretically resulting in an infinite number of copies of the original.  In others we slightly alter the goal so that the initial assembly to be replicated contains additional information in the form of a ``tag'' (i.e. an appended line of tiles) which specifies the exact number of copies to be created.

\subsection{Exponentially speeding up, unbounded replication}

[Describe the ``environment'', input, and output in technical terms]

%[Describe the class(es) of shapes handled.  For basic replication the only restriction may be that all features have width $\ge 2$ (or actually $4$?), although we may still need a specially designated corner and I'm not sure how to find that without the restriction that concavities can't ``turn''.]

%[Describe the construction:  (1) create a frame, (2) upon completion of the frame it detaches, (3) an inner ring forms within the ring, (4) upon completion the tiles of the inner ring are swapped out, (5) the outer ring detaches and is free to make another copy, while the interior of the inner ring fills in and and assembly can also host the growth of another new ring.]

The next theorem states that we can replicate any hole-free connected shape an unbounded number of times.  Our proof of this theorem is by construction.  We now provide a high level overview of the construction.  Let $P$ be a connected hole free shape.  Our construction begins with designing a tile set that builds a frame around $P$ which detaches upon completion.  Next, we design tiles so that an inner ring forms within the completed ring.  Once this ring within a ring is complete, it detaches and fills in its interior.  The outer ring is then free to make another copy while the interior of the inner ring can host the growth of another ring.

\begin{theorem}\label{thm:exp_rep}
There exists an STAM tile set at temperature $2$ which can infinitely replicate any hole-free connected shape $P$.
\end{theorem}

We now present a proof sketch of Theorem~\ref{thm:exp_rep}.  Let $P$ be a connected shape in $\mathbb{N}^2$.  Our construction begins with building a frame around the shape $P$ using the machinery from the previous sections.  We design our tile set for this frame system so that once the frame completes, it detaches from the shape $P$.  Furthermore, we design the tile set of this system, so that 1) there exists exactly one south east corner of the frame which exposes a $z$ glue on the north of the west most tile and a $y$ glue on the west side of the north most tile and 2) on every other interior side of the frame, a $y$ and an $N$ glue is exposed.  An example of such a frame is shown in Figure~\ref{fig:rep_frame_ex}.  We refer to this frame as the outer frame.

\begin{figure}[htp]
\centering
    \includegraphics[width=2.0in]{images/rep_frame_ex}
    \caption{An example of the glues lining the interior of a frame.}
    \label{fig:rep_frame_ex}
\end{figure}

To construct the set of tiles which forms an inner ring inside the previously constructed ring, we begin by adding the tile shown in Figure~\ref{fig:rep_start_tile}.  Notice that this tile will bind to our specially selected south east corner and propagate a $w$ signal to the north.  If there is not a tile north of the tile which initiates the growth of the inner frame, the tile shown in Figure~\ref{fig:rep_north_crawler} will cooperatively bind to the $y$ glue outer frame and the $w$ glue of the tile shown in Figure~\ref{fig:rep_start_tile}.  We call this tile the north crawler tile.  Once the north crawler tile binds, it will present two glues, an $E$ glue and an $N$ glue.  If a tile does not lie to the west of the north crawler tile, a \emph{primer tile} (shown in Figure~\ref{fig:rep_primer}) will attach to the $E$ glue on the west of the north crawler tile and turn on the glues as indicated in Figure~\ref{fig:rep_north_crawler}.  This allows for the $w$ signal to propagate north.  Upon attachment of the primer tile, the north crawler tile turns off its $E$ glue and turns on an $N$ glue.  Note that the $E$ glue is a strength 2 glue.  If there is a tile to the west of the north crawler gadget, the $N'$ glue will bind to the $N$ glue of the outer frame and turn on the glues indicated in Figure~\ref{fig:rep_north_crawler}.  Note that that once a north crawler tile binds to the outer frame, it is guaranteed that either its $N$ glue will be ``fired'' or its ``E'' glue will be fired.  Also, observe that the only difference in the glues triggered by these two glues is the $E$ glue turns on the $w'$ glue on the west side of the north crawler tile and the $N$ glue.  The $N$ glue will allow south crawler tiles (a reflected version of the north crawler tile which propagates the $w$ signal south) to ``bounce'' signals so that they can continue grow.  The $w'$ glue will allow for the propagation of the $w$ signal in the event that the inner ring that is forming crashes into itself.

North crawler tiles will continue to attach until 1) there is no longer a $y$ glue to which the north crawler tile can cooperatively bind or 2) the attachment of the north crawler tile is prevented by a tile existing in the outer frame.  In the case of 1, we add the two tiles shown in Figure~\ref{rep_north_duple} which we think of as being preformed and binding cooperatively with the propagated $w$ signal and the $y$ glue of the outer frame.  Once this ``duple'' binds, an $E$ and an $N$ glue can bind to either a primer tile or a tile from the outer frame, respectively, which will start the propagation of a $w$ signal to the east.  Note that if either $E$ glue is ``triggered'', a $w'$ glue will be exposed on the west and/or north of the duple.

In the case of 2, the $y'$ glue on the top of the north crawler tile will ``bounce'' off of the $y$ glue on the outer frame tile which is preventing it from continuing and start propagating the $w$ signal west.  Furthermore,  if there is also a tile to the west of this north crawler tile, the $w$ signal will ``bounce'' off of the outer frame tile which lies to the west and begin propagating southward.

To complete the frame, we add rotated versions of each of the tiles discussed so far (except for the start tile) so that the $w$ signal may be propagated to the north, east, west, and south of the frame in a counterclockwise fashion.

\begin{figure}[htp]
\centering
    \includegraphics[width=2.0in]{images/rep_start_tile}
    \caption{The tile which begins the growth of the inner frame.}
    \label{fig:rep_start_tile}
\end{figure}

\begin{figure}[htp]
\centering
    \includegraphics[width=2.0in]{images/rep_north_crawler}
    \caption{The tile which propagates the $w$ signal to the north.}
    \label{fig:rep_north_crawler}
\end{figure}

\begin{figure}[htp]
\centering
    \includegraphics[width=1.0in]{images/rep_primer}
    \caption{A primer tile which allows for the $w$ signal to propagate to the north and turns on a $w'$ glue on the west side of the north crawler tile.}
    \label{fig:rep_primer}
\end{figure}

\begin{figure}[htp]
\centering
    \includegraphics[width=4.0in]{images/rep_north_duple}
    \caption{The ``duple'' which allows the $w$ signal to propagate to the east when there is not a $y$ glue for the north crawler tile to cooperatively bind to.}
    \label{fig:rep_north_duple}
\end{figure}

We now modify the tiles discussed above, so that 1) the inner frame separates from the outer frame, 2) the inner frame fills its interior with tiles and 3) the inner frame exposes $x$ glues along its border like the original shape.  To allow the inner frame to detach, we overlay signals on all of the tiles which turn off all of the $y'$ glues on the inner frame.  We add these signals so that this cascade of signals is triggered once the $w$ signal reaches the start tile.  To ensure we do not have any extra exposed glues after our frame detaches, we add these signals so that they follow the $w$ signal as seen in previous sections.  To fill in the shape, we modify the glues turned on by the $E$ glue to include a strength $1$ glue which we call $fill_1$.  In addition, we overlay signals on all the tiles so that when the frame completes, a strength $1$ glue which we call $fill_2$ is exposed on all sides of all tiles in the inner frame which started off with an $E$ glue.  We overlay these signals using the signal following technique mentioned above so that no $fill_2$ glues are exposed on the exterior of the frame.  Now notice that we can design ``filler'' tiles which bind using glues $fill_1$ and $fill_2$ and blindly fill in the interior of the inner frame.  Next, we can add extra signals to the $y'$ glues on the tiles in the inner frame so that when the $y'$ glues ``bounces'' off the $y$ glue on the outer frame, it exposes an $x$ glue on the same side of the tile as it is located.

\subsubsection{Frame Example}
Figure~\ref{fig:rep_examples} shows a schematic diagram of the propagation of the $w$ signal.  Notice that the $w$ signal always attempts to take the counterclockwise most path.  It does this by ``bouncing'' off of glues of existing tiles until it finds an edge which does not have a tile abutting it.  Also, note that in all examples shown in Figure~\ref{fig:rep_examples} the $w$ signal is able to pass through existing tiles in the inner frame because the primer tiles have turned on the $w'$ glue which allows for the tile to ``receive'' the $w$ signal.
\begin{figure}[htp]
\centering
  \subfloat[][]{%
        \label{fig:rep_examples1}%
        \makebox[1.6in][c]{\includegraphics[width=1.5in]{images/rep_examples1}}
        }%
        \quad\quad
  \subfloat[][]{%
        \label{fig:rep_examples2}%
        \makebox[1.6in][c]{\includegraphics[width=1.7in]{images/rep_examples2}}
        }%
        \quad\quad
  \subfloat[][]{%
        \label{fig:rep_examples3}%
        \makebox[1.6in][c]{\includegraphics[width=1.7in]{images/rep_examples3}}
        }%
  \caption{A schematic view of how the $w$ signal is passed through the inner frame.  The darkly shaded tiles represent the outer frame and the lightly shaded tiles represent the tiles composing the inner frame.  The path through the tiles indicates the flow of the $w$ signals through the inner frame.}
  \label{fig:rep_examples}
\end{figure}

\subsubsection{Proof of Correctness}
To see that the construction is correct we first show that the $w$ signal is always able to travel counterclockwise around the ring and end back at the tile which initiated the growth of the inner ring.  For this, we consider two cases: 1) all ``corridors'' in the interior of the outer frame are at least two tiles wide and 2) there are ``corridors'' in the interior of the outer frame which are only one tile wide. In case 1, notice that the $w$ signal never has to ``loop'' back onto a tile which previously propagated it.  The $w$ signal propagates through tiles placed in a clockwise fashion until it arrives at the start tile.  Once this occurs, we are done.

In the second case, we assume there are ``corridors'' in the interior of the outer frame which are only one tile wide.  Notice, that by the design of our tile set after tiles fill the corridor, the tile which started the propagation of $w$ into the single tile wide corridor will once again receive the $w$ signal and propagate it in a counterclockwise fashion.  Thus, we can apply the argument for case 1 to see that the $w$ signal will propagate until it reaches the start tile.

Once the inner frame detaches from the outer frame, we must ensure that the inner frame cannot inadvertently bind to other assemblies in the system.  To see this, note that after detachment, the inner frame can only have $w$ and $E'$ glues exposed and at most either a $y'$ glue, $z'$, or $N'$ glue exposed.
%\subsection{Precisely bounded replication}
%
%[Describe the ``tag'' for input assemblies.]
%
%[Describe the construction: A relatively slight modification of the previous so that the frame begins on the tag, which represents $n$, then creates a copy of the assembly with a tag containing $n-1$.  If the tag represents $0$, no tag is attached to the new copy.  Since replication can only begin from tags, it halts.]


==> replication2.tex <==
\vspace{-10pt}
\section{Replication} \label{sec:rep}
In this section, we provide a construction in the STAM which is capable of replicating the shapes of a given set of input assemblies with the restriction that the shapes of the input assembly cannot be disconnected by removing a single tile, i.e. shapes with minimum width (\emph{min-width}) 2.  Furthermore, we show this replication can be done in an exponential manner.
\vspace{-12pt}
\subsection{Exponential, unbounded replication}
We now define what it means for an STAM system to replicate a shape $P$.  In the following definition, we assume that the input assemblies $\sigma_1, \sigma_2, ..., \sigma_n$ all have the same glue on each edge of their perimeter and there is only one of each in the system.  We say that an STAM system $\mathcal{T} = (T, \{\sigma_1, \sigma_2, ..., \sigma_n\}, \tau)$ infinitely replicates the shapes $P_1, P_2, ..., P_n$ provided that 1) $\dom{\sigma_i} = P_i$ for all $i$, 2) there are a bounded number of different terminal assemblies, and 3) there are an infinite number of assemblies of shape $P_i$ for all $i$.  We call assemblies $\sigma_1, \sigma_2, ..., \sigma_n$ replicable supertiles.  In general, a replicable supertile in a system $\mathcal{T}$ is a supertile which can be ``replicated''.

In the replication process for a shape $P$, we consider a time step to be producing a new assembly $\alpha$ with $\dom{\alpha} = P$.  We say that an STAM system $\mathcal{T}$ \emph{exponentially replicates without bound} the shapes $P_1, P_2, ..., P_n$ provided that 1) the system $\mathcal{T}$ infinitely replicates the shapes $P_1, P_2, ..., P_n$, 2) the number of (super)tile attachment and/or detachments required in the creation of a copy of shape $P_i$ (i.e. one time step) is bounded by $poly(|P_i|)$, 3)
every (super)tile attachment involves a singleton tile or a two tile assembly and an existing assembly that is replicating $P_i$ for some $i$ (i.e. tiles either attach to a frame layer or attach as filler tiles); and moreover, all supertile detachment involves either a single tile wide rectangle detaching from a frame, a completed frame detaching from a seed shape assembly $P_i$ for some $i$, or a completed frame detaching from a replicated shape assembly $P_i$ for some $i$, and 4) if there are $n$ copies of the shape $P_i$ at time step $t$, then there are $2n$ copies of the shape $P_i$ at time step $t+1$. Though this definition is specific to the replication technique given by our construction, it is motivated by the observation that for a single shape $P$, if a system $\mathcal{T}$ exponentially replicates without bound the shape $P$, then $\mathcal{T}$ exponentially replicates the shape $P$ according to the more general definition of exponential replication given in~\cite{SignalsReplication} (Definition 3).

\begin{theorem}\label{thm:exp_rep}
For any finite set of hole-free, min-width $2$ shapes $P$ $=$ $\{P_1, P_2, ...,$ $ P_n\}$, there exists an STAM system $\calT = (T, \sigma_P, 2)$, with $\sigma_P$ a set of $n$ assemblies, one of each shape in $P$, and $\calT$ exponentially replicates without bound all shapes in $P$.

\end{theorem}

We now provide a high level overview of the construction.  Let $P$ be a connected, hole-free, min-width $2$ shape.  Our construction begins with designing a tile set that builds a frame around $\sigma$ where $\dom(\sigma) = P$ which detaches upon completion.  Next, we design tiles so that an inner ring forms within the completed ring.  Once this ring within a ring is complete, it detaches and fills in its interior.  The outer ring is then free to make another copy while the interior of the inner ring can host the growth of another frame.

Our construction begins with adding tiles to our tile set which build a frame around $\sigma$ using the machinery from the previous sections.  We design our tile set for this frame system so that once the frame completes, it detaches from $\sigma$ with (1) exactly one south east corner of the frame which exposes a $z$ glue on the north of the west most tile and a $y$ glue on the west side of the north most tile of that corner, and (2) on every other interior side of the frame, a $y$ glue is exposed.  We refer to this frame as the outer frame.

To construct the set of tiles which forms an inner ring inside the outer frame, we begin by adding to our tile set the tiles shown in Figure~\ref{fig:rep_tiles}. \vspace{-20pt}

\begin{figure}[htp]
\centering
  \subfloat[][The tile which begins the growth of the inner frame.]{%
        \label{fig:rep_start_tile-main}%
	        \includegraphics[width=0.75in]{images/rep_start_tile2}
        }%
        \quad\quad
  \subfloat[][A north crawler tile which propagates the $w$ signal north.]{%
        \label{fig:rep_north_crawler-main}%
        		\includegraphics[width=0.75in]{images/rep_north_crawler2}
        }%
        \quad\quad
  \subfloat[][The ``duple'' which allows the $w$ signal to propagate to the east when there is not a $y$ glue for a north crawler tile to cooperatively bind to.]{%
        \label{fig:rep_north_duple-main}%
        		\includegraphics[width=1.5in]{images/rep_north_duple2}
        }%
        \quad\quad
  \subfloat[][The ``filler'' tile.]{%
        \label{fig:rep_filler}%
                \includegraphics[width=0.8in]{images/rep_filler}
        }%
  \caption{The partial tile set which builds an inner frame and fills it.\vspace{-15pt}}
  \label{fig:rep_tiles}
\end{figure}

To complete the tile set for the inner frame, we add rotated versions of each of the tiles discussed so far to $T$ (except for the start tile) so that the $w$ signal may be propagated to the north, east, west, and south of the frame in a counterclockwise fashion.

We now modify the tiles discussed above, so that (1) the inner frame separates from the outer frame, (2) the inner frame fills its interior with tiles and (3) the inner frame exposes $x$ glues along its border like the original shape.  To allow the inner frame to detach, we overlay signals on all of the tiles which turn off all of the $y'$ glues on the inner frame.  We add these signals so that this cascade of signals is triggered once the $w$ signal reaches the start tile.  To ensure we do not have any extra exposed glues after our frame detaches, we add these signals so that they follow the $w$ signal (see\ifinproceedings~\cite{STAMshapes-arxiv} \else Section~\ref{sec:signal-following}\fi for signal following gadgetry).  To fill in the shape, we once again overlay signals on the existing tile set so that when the signal returns to the initial tile, it initiates a signal which exposes strength $2$ \emph{fill} glues allowing for the attachment of ``filler tiles'' on the interior of the inner frame.  These filler tiles simply attach and trigger signals on all $3$ remaining sides which allow for the attachment of more filler tiles.  Next, we add signals to the $y'$ glues on the tiles in the inner frame so that when a $y'$ glue attaches to a $y$ glue on the outer frame, it activates an $x$ glue on the same side.
\vspace{-15pt}
\subsubsection{Frame example}
Figure~\ref{fig:rep_examples-main} shows a schematic diagram of the propagation of the $w$ signal.  Notice that the $w$ signal always attempts to take the counterclockwise most path.  It does this by ``bouncing'' off of glues of existing tiles until it finds an edge which does not have a tile abutting it.
\begin{figure}[htp]
\vspace{-25pt}
\centering
  \subfloat[][]{%
        \label{fig:rep_examples21}%
        \makebox[1.4in][c]{\includegraphics[width=1.5in]{images/rep_examples21}}
        }%
        \quad\quad
  \subfloat[][]{%
        \label{fig:rep_examples22}%
        \makebox[1.4in][c]{\includegraphics[width=1.3in]{images/rep_examples22}}
        }%
  \caption{A schematic view of how the $w$ signal is passed through the inner frame.  The darkly shaded tiles represent the outer frame and the lightly shaded tiles represent the tiles composing the inner frame.  The path through the tiles indicates the flow of the $w$ signals through the inner frame. \vspace{-5pt}}
  \label{fig:rep_examples-main}
\end{figure}

\subsubsection{Exponential, unbounded replication of shapes at scale factor $2$}
Since all shapes at scale factor $2$ are min-width $2$ shapes, Theorem~\ref{thm:exp_rep} yields the following corollary.

\begin{corollary}

For any finite set of hole-free shapes $P = \{P_1, P_2, ..., P_n\}$, let $P' = \{P'_1, P'_2, ..., P'_n\}$ be the shapes of $P$ at scale factor $2$. Then, there exists an STAM system $\calT = (T, \sigma_P', 2)$, with $\sigma_P'$ a set of $n$ assemblies, one of each shape in $P'$, and $\calT$ exponentially replicates without bound all shapes in $P'$.

%Let $P_1, P_2, ..., P_n$ be hole-free connected shapes and let $P'_1, P'_2, ..., P'_n$ be the shapes $P_1, P_2, ...,P_n$ at scale factor $2$.  Then, there exists an STAM tile set at temperature $2$ which exponentially replicates $P'_1, P'_2, ..., P'_n$ without bound.
\end{corollary}

\ifabstract
\later{
\section{Replication} \label{sec:rep_app}

In this section, we provide a construction in the STAM which is capable of replicating the shapes of a given set of input assemblies with the restriction that the shapes of the input assemblies cannot be disconnected by removing a single tile.  We call such shapes min-width $2$ shapes.  Furthermore, we show this replication can be done in an exponential manner.


\subsection{Exponential, unbounded replication}
We now define what it means for an STAM system to replicate a shape $P$.  In the following definition, we assume that the input assemblies $\sigma_1, \sigma_2, ..., \sigma_n$ all have the same glue on each edge of their perimeter and there is only one of each in the system.  We say that an STAM system $\mathcal{T} = (T, \{\sigma_1, \sigma_2, ..., \sigma_n\}, \tau)$ infinitely replicates the shapes $P_1, P_2, ..., P_n$ provided that 1) $\dom{\sigma_i} = P_i$ for all $i$, 2) there are a bounded number of different terminal assemblies, and 3) there are an infinite number of assemblies of shape $P_i$ for all $i$.  We call assemblies $\sigma_1, \sigma_2, ..., \sigma_n$ replicable supertiles.  In general, a replicable supertile in a system $\mathcal{T}$ is a supertile which can be ``replicated''.

In the replication process for a shape $P$, we consider a time step to be producing a new assembly $\alpha$ with $\dom{\alpha} = P$ for all replicable supertiles currently in the system.  We say that an STAM system $\mathcal{T}$ \emph{exponentially replicates without bound} the shapes $P_1, P_2, ..., P_n$ provided that 1) the system $\mathcal{T}$ infinitely replicates the shapes $P_1, P_2, ..., P_n$, 2) the number of (super)tile attachment and/or detachments required in the creation of a copy of shape $P_i$ (i.e. one time step) is bounded by $poly(|P_i|)$, 3) every (super)tile attachment involves a singleton tile or a two tile assembly and an existing assembly that is replicating $P_i$ for some $i$ (i.e. tiles either attach to a frame layer or attach as filler tiles); and moreover, all supertile detachment involves either a single tile wide rectangle detaching from a frame, a completed frame detaching from a seed shape assembly $P_i$ for some $i$, or a completed frame detaching from a replicated shape assembly $P_i$ for some $i$, and 4) if there are $n$ copies of the shape $P_i$ at time step $t$, then there are $2n$ copies of the shape $P_i$ at time step $t+1$. Though this definition is specific to the replication technique given by our construction, it is motivated by the observation that for a single shape $P$, if a system $\mathcal{T}$ exponentially replicates without bound the shape $P$, then $\mathcal{T}$ exponentially replicates the shape $P$ according to the more general definition of exponential replication given in~\cite{SignalsReplication} (Definition 3).

We say that a shape $P$ is a min-width $2$ shape provided that two conditions hold: 1) if $\vec{v} = (v_1, v_2) \in \dom{(P)}$, then either $(v_1-1, v_2) \in \dom{(P)}$ or $(v_1+1, v_2) \in \dom{(P)}$ and 2) if $\vec{v} = (v_1, v_2) \in \dom{(P)}$, then either $(v_1, v_2 - 1) \in \dom{(P)}$ or $(v_1, v_2+1) \in \dom{(P)}$.  Intuitively, we can think of this as the set of shapes which cannot be disconnected by removing a single tile.

%[Describe the construction:  (1) create a frame, (2) upon completion of the frame it detaches, (3) an inner ring forms within the ring, (4) upon completion the tiles of the inner ring are swapped out, (5) the outer ring detaches and is free to make another copy, while the interior of the inner ring fills in and and assembly can also host the growth of another new ring.]

The next theorem states that we can exponentially replicate without bound any hole-free, connected, min-width $2$ shape.  Our proof of this theorem is by construction.  We now provide a high level overview of the construction.  Let $P$ be a connected, hole-free, min-width $2$ shape.  Our construction begins with designing a tile set that builds a frame around $P$ which detaches upon completion.  Next, we design tiles so that an inner ring forms within the completed ring.  Once this ring within a ring is complete, it detaches and fills in its interior.  The outer ring is then free to make another copy while the interior of the inner ring can host the growth of another ring.

\begin{theorem}\label{thm:exp_rep}
There exists an STAM tile set at temperature $2$ which exponentially replicates without bound any set of min-width $2$ shapes $P_1, P_2, ..., P_n$.
\end{theorem}

We now present a proof sketch of Theorem~\ref{thm:exp_rep}.  We show the theorem holds when $n=1$ (that is, there is only one input assembly shape to be replicated), and note that it easily generalizes to $n>1$.   Let $P$ be a hole-free, connected, min-width $2$ shape in $\mathbb{N}^2$ which has component size $2$.  We create a system $\mathcal{T} = (T, \sigma, 2)$ where $T$ is the tile set we describe throughout the construction and $\sigma$ is an assembly with $\dom(\sigma) = P$ whose perimeter tiles all expose a glue $x$.  Our construction begins with adding tiles to $T$ which build a frame around $\sigma$ using the machinery from the previous sections.  We design our tile set for this frame system so that once the frame completes, it detaches from $\sigma$.  Furthermore, we design the tile set of this system, so that 1) there exists exactly one south east corner of the frame which exposes a $z$ glue on the north of the west most tile and a $y$ glue on the west side of the north most tile and 2) on every other interior side of the frame, a $y$ glue is exposed.  An example of such a frame is shown in Figure~\ref{fig:rep_frame_ex}.  We refer to this frame as the outer frame.

\begin{figure}[htp]
\centering
    \includegraphics[width=2.0in]{images/rep_frame_ex2}
    \caption{An example of the glues lining the interior of a frame.}
    \label{fig:rep_frame_ex}
\end{figure}

To construct the set of tiles which forms an inner ring inside the previously constructed ring, we begin by adding to $T$ the tile shown in Figure~\ref{fig:rep_start_tile} which we call the start tile.  Notice that this tile will bind to our specially selected south east corner and propagate a $w$ signal to the north.  Next, we add the tile shown in Figure~\ref{fig:rep_north_crawler} to $T$ which will cooperatively bind to the $y$ glue of the outer frame and the $w$ glue of the tile shown in Figure~\ref{fig:rep_start_tile}.  We call this tile the north crawler tile.  North crawler tiles will continue to attach until 1) there is no longer a $y$ glue to which the north crawler tile can cooperatively bind or 2) the attachment of the north crawler tile is prevented by a tile existing in the outer frame.  In the case of 1, we add the two tiles shown in Figure~\ref{fig:rep_north_duple} to $T$ which we think of as being preformed and binding cooperatively with the propagated $w$ signal and the $y$ glue of the outer frame.  Once this ``duple'' binds, it will start the propagation of a $w$ signal to the east.  In the case of 2, the $y'$ glue on the top of the north crawler tile will ``bounce'' off of the $y$ glue on the outer frame tile which is preventing it from continuing and start propagating the $w$ signal west.

To complete the tile set for the inner frame, we add rotated versions of each of the tiles discussed so far to $T$ (except for the start tile) so that the $w$ signal may be propagated to the north, east, west, and south of the frame in a counterclockwise fashion.

We now modify the tiles discussed above, so that 1) the inner frame separates from the outer frame, 2) the inner frame fills its interior with tiles and 3) the inner frame exposes $x$ glues along its border like the original shape.  To allow the inner frame to detach, we overlay signals on all of the tiles which turn off all of the $y'$ glues on the inner frame.  We add these signals so that this cascade of signals is triggered once the $w$ signal reaches the start tile.  To ensure we do not have any extra exposed glues after our frame detaches, we add these signals so that they follow the $w$ signal as seen in previous sections.  To fill in the shape, we once again overlay signals on the existing tile set so that when the signal returns to the initial tile, the initial tile sends out a signal which exposes strength $2$ glues which allow for the attachment of ``filler tiles''.  These filler tiles simply attach, and trigger signals on all $3$ remaining sides which allow for the attachment of more filler tiles.  Next, we can add extra signals to the $y'$ glues on the tiles in the inner frame so that when the $y'$ glues ``bounces'' off the $y$ glue on the outer frame, it exposes an $x$ glue on the same side of the tile as it is located.

\begin{figure}[htp]
\centering
    \includegraphics[width=1.5in]{images/rep_start_tile2}
    \caption{The tile which begins the growth of the inner frame.}
    \label{fig:rep_start_tile}
\end{figure}

\begin{figure}[htp]
\centering
    \includegraphics[width=1.5in]{images/rep_north_crawler2}
    \caption{The tile which propagates the $w$ signal to the north.}
    \label{fig:rep_north_crawler}
\end{figure}

\begin{figure}[htp]
\centering
    \includegraphics[width=2.5in]{images/rep_north_duple2}
    \caption{The ``duple'' which allows the $w$ signal to propagate to the east when there is not a $y$ glue for the north crawler tile to cooperatively bind to.}
    \label{fig:rep_north_duple}
\end{figure}

\begin{figure}[htp]
\centering
        \includegraphics[width=1.5in]{images/rep_filler}
        \caption{The ``filler'' tile.}
        \label{fig:rep_filler}
\end{figure}


\subsubsection{Frame example}
Figure~\ref{fig:rep_examples} shows a schematic diagram of the propagation of the $w$ signal.  Notice that the $w$ signal always attempts to take the counterclockwise most path.  It does this by ``bouncing'' off of glues of existing tiles until it finds an edge which does not have a tile abutting it.
\begin{figure}[htp]
\centering
  \subfloat[][]{%
        \label{fig:rep_examples21}%
        \makebox[1.6in][c]{\includegraphics[width=1.5in]{images/rep_examples21}}
        }%
        \quad\quad
  \subfloat[][]{%
        \label{fig:rep_examples22}%
        \makebox[1.6in][c]{\includegraphics[width=1.7in]{images/rep_examples22}}
        }%
  \caption{A schematic view of how the $w$ signal is passed through the inner frame.  The darkly shaded tiles represent the outer frame and the lightly shaded tiles represent the tiles composing the inner frame.  The path through the tiles indicates the flow of the $w$ signals through the inner frame.}
  \label{fig:rep_examples}
\end{figure}

\subsubsection{Proof of correctness}
We now show that the system $\mathcal{T}$ described above exponentially replicates without bound the shape $P$.  To see this, we first argue that the system infinitely replicates the shape $P$, and then we show that the system exponentially replicates $P$ without bound.

It is straight forward to see that the $w$ signal always returns to the start tile, and consequently that the frame detaches and fills in.  Note that this implies that there will be an infinite number of $\alpha$ assemblies in $\mathcal{A}_{\Box}[\mathcal{T}]$ with the property that $\dom{\alpha} = P$.   Thus, we show that after the inner frame detaches from the outer frame, it cannot inadvertently bind to another assembly in the system which will show that there are only a bounded number of terminal assemblies in the system.  To see this, note that the only glues exposed on the outside of the inner frame after it detaches are $w$ and $x$ glues and one $z$ glue.  But, this is not an issue because there are not any assemblies in the system which expose more than one $w'$ glue or $z'$ glue.  Consequently, the $w$ glues cannot allow for the attachment of other assemblies.

To see that this replication occurs in an exponential manner, note that after each inner frame detaches, they expose $x$ glues which will allow another frame to begin to form.  Thus, if at time step $t-1$ there are $n$ replicable supertiles, at time step $t$ there will be $2n$ replicable supertiles. Hence, conditions 1 and 4 in the definition of exponential replication without bound holds. Moreover, note that in the assembly of a completed frame, the assembly of each frame layer requires $O(|P|)$ tile attachments and there $O(|P|)$ frame layers are required to complete a frame, which satisfies condition 2. Finally, by construction, condition 3 holds. Consequently, $\mathcal{T}$ exponentially replicates $P$ without bound.

} %later
\fi

